Objects do not disappear: Video object detection by single-frame object location anticipation

Objects in videos are typically characterized by continuous smooth motion. We exploit continuous smooth motion in three ways. 1) Improved accuracy by using object motion as an additional source of supervision, which we obtain by anticipating object locations from a static keyframe. 2) Improved efficiency by only doing the expensive feature computations on a small subset of all frames. Because neighboring video frames are often redundant, we only compute features for a single static keyframe and predict object locations in subsequent frames. 3) Reduced annotation cost, where we only annotate the keyframe and use smooth pseudo-motion between keyframes. We demonstrate computational efficiency, annotation efficiency, and improved mean average precision compared to the state-of-the-art on four datasets: ImageNet VID, EPIC KITCHENS-55, YouTube-BoundingBoxes, and Waymo Open dataset. Our source code is available at https://github.com/L-KID/Videoobject-detection-by-location-anticipation.

==> Paper/experiments_bkp.tex <==
\section{Experiments}
\noindent\textbf{Datasets and evaluation setup.}
We test our hypotheses on a fully controlled MovingDigits dataset. 
We ablate model choices on a subset of ImageNet VID~\cite{ILSVRC15}. 
We show the practical benefits of our approach on the full ImageNet VID~\cite{ILSVRC15} and on EPIC KITCHENS-55~\cite{damen2018scaling}. 
As a realistic sparsely annotated dataset we evaluate on YouTube-BoundingBoxes ~\cite{real2017youtube}, which has approximately 1 keyframe annotation per second.
For the ImageNet VID experiments, we train our model on a combination of ImageNet VID and DET datasets as a common practice in \cite{wu2019sequence, zhu2017flow, cui2021tf, han2020mining}. 
To quantify detection accuracy we adopt the common approach ~\cite{chen2020memory,cui2021tf,wang2018fully,wu2019sequence} by computing mean Average Precision (mAP), where a detection is correct if its Intersection over Union (IoU) with the ground truth is sufficiently large. 
Note that although our method samples keyframes during training, we evaluate on all frames at test time, unless stated otherwise.

%---------------------------------------------------------------
\smallskip\noindent\textbf{Implementation details.}
We use Faster R-CNN \cite{ren2015faster} with an ImageNet pre-trained ResNet base as the object detection backbone. %, but any other object detector choice is equally applicable.
%In the Faster R-CNN the RPN head is added on the top of \textit{conv5} stage.
% We add our module by two fully connected layers upon the RoI pooled features, followed by classification and bounding box regression \slp{Do we change the Faster R-CNN architecture, why?}.
Our trajectory prediction sub-network contains three fully-connected layers with 1024 dimensions for the middle layer, see \fig{overview}. 
% \fkn{You could also mention what is in each batch. Does the batch contain all the keyframes or subset of keyframes or just one individual keyframe. Do you use other video clips in the batch? What is the length of each clip? Something like: The batch consists of the keyframes of a clip as a part of the batch together with other keyframes of different clips. The training can also handle one frame per clip every time. Each clip contains x seconds of video for EpicKitchen and y seconds for ImageNet Vid. We tested 4 and 8 keyframes.}
We train our network for 120k iterations on ImageNet VID and 173k iterations on Epic Kitchens with the SGD optimizer, on 4 GPUs.
For ImageNet VID, the initial learning rate is \num{e-3} and is divided by 10 at 80K iterations.
For Epic Kitchens, the initial learning rate is \num{5e-4} and is divided by 10 at 120K iterations.
For YouTube-BoundingBoxes, the initial learning rate is \num{5e-4} and is divided by 10 at 100k iterations.

%=========================================================================================
\subsection{Hypothesis testing}

We test our hypotheses by creating a fully controlled dataset, MovingDigits, where we pair each of the 10 MNIST digit classes with a unique, linear motion of 2px per frame, see \fig{h1}.
Each video has 32 frames with a frame size of 64$\times$64 px.
We created 200 videos for training and 80 videos for testing, with an equal number of videos per class. We use a trajectory length of $T{=}8$, train for  1.25k iterations and use a ResNet-18 feature extractor.

\medskip\noindent\textbf{[H1]: Can the model anticipate motion trajectories?}
To verify if our model can anticipate trajectories from a single static input frame $t$, we train on MovingDigits, where each digit has its own linear motion. We calculate the average IoU over the predicted trajectories for the test videos. The IoU is 0.95, which is near-perfect compared to the IoU of 0.79 for no motion anticipation. We show an example of the predicted bounding boxes (Bbox) by our method and the ground truth bounding boxes (GT Bbox) from time steps $t$ to $t+3$ in \fig{h1}. %We can see our predicted bounding boxes match the ground truth boxes, and move in the same direction. 
We conclude that our model can successfully learn motion by anticipating trajectories from a static input frame. 

%We create a test set containing digits moving in different directions compared to the actual MovingDigits test set. We refer to this new test set as \textsc{Test-diff}, and to the original MovingDigits test set as . Given the small dataset size, here we use a ResNet-18 backbone, pre-trained on ImageNet, and finetune the complete model on MovingDigits with both test sets \textsc{Test} and \textsc{Test-diff}.\slp{What do you mean you finetune on the test sets?! Did you mean you evaluate on them?}

%\fig{h1} visualizes two sets of videos from class 6 and class 4. Digit 6 moves in the direction top-left, and digit 4 moves bottom-left in the training set of MovingDigits and in the \textsc{Test} set. However, in the \textsc{Test-diff} we changed the directions such that digit 6 moves to the right and digit 4 moves bottom-right. 
%The left column shows that digit 6 class moves in the up-left direction, and digit 4 class moves to the bottom-left in the training set.
%The middle column shows that digits move in the same directions with that in the training set for the original MovingDigits test set \textit{Test}.
%And the bounding box detection moves following the digits.
%The right column shows that digit 6 moves to the right, and digit 4 moves to the bottom-right, where the moving directions differ from the training set.
%The results show that the box predictions of digits 6 and 4 in the \textsc{Test} video follow, as expected, the direction of digits in the training set.
%However, on the \textsc{Test-diff} instead of following the actual digits, the box detections still follow the training set directions: \ie top-left for digit 6 and and bottom-left for digit 4.
%Similarly, the bounding box detection of digit 4 in the test video also moves in the same direction with that in the training set.
%Our method indeed learns to associate a specific object appearance with a specific motion pattern.

% \begin{figure}
%     \centering
%     \begin{tabular}{ccc}
%     \small{Input frame} & \small{GT Bbox} & \small{Predicted Bbox} \\
%     \includegraphics[width=0.3\linewidth]{Images/video_6_keyframe.pdf} & 
%     \includegraphics[width=0.3\linewidth]{Images/video_6_gtBbox_wDigit.pdf} &
%     \includegraphics[width=0.3\linewidth]{Images/video_6_same3.pdf} \\
%     \includegraphics[width=0.3\linewidth]{Images/video_4_keyframe.pdf} &
%     \includegraphics[width=0.3\linewidth]{Images/video_4_gtBbox_wDigit.pdf} &
%     \includegraphics[width=0.3\linewidth]{Images/video_4_same3.pdf} \\
%     $t$ & $t+1 \colon t+4$ & $t+1 \colon t+4$ 
%     \end{tabular}
%     \caption{ 
%     \textbf{[H1]: Trajectory anticipating on MovingDigits.} We show time-accumulated frames of digits 6 and 4. Each digit class has an associated linear motion (green arrow). We evaluate trajectory forecasting from a single image on the \textsc{Test-simil} videos where the motion is similar to the training videos, and on the \textsc{Test-diff} videos which have different motion than trained on.  Computing the average IoU@[0.50:.05:0.95] for the forecasts (orange boxes) shows that our model can predict trajectories from a static frame, if similar trajectories are observed in the training set. 
%     %The moving directions of digit 6 and digit 4 as well as their bounding-box detection are the same with that in the training. 
%     %The moving directions of digit 6 and digit 4 are different from that in the training set. 
%     %Regardless of the test set, the bounding-box predictions still follow the directions the corresponding digits have in the training set. 
%     %Our model learns to associate object appearance with motion. 
%     %\fkn{The figure is beautiful. However, it is a bit confusing if you don't read the caption. For example, for digit 4 is it not clear the digit moves in the same direction as of the training set. If you get time, you may change the figure with the trajectory line.}
%     \slp{I do not think for GT and Predicted the boxes the digit should be moving cause now it's tracking. See fig1.}
%     }
%     \label{fig:h1}
% \end{figure}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}
%     \centering
%     \begin{tabular}{ccc}
%     \small{Input frame} & \small{GT Bbox} & \small{Predicted Bbox} \\
%     \includegraphics[width=0.3\linewidth]{Images/video_6_keyframe.pdf} & 
%     \includegraphics[width=0.3\linewidth]{Images/video_6_gtBbox_arrow.pdf} &
%     \includegraphics[width=0.3\linewidth]{Images/video_6_dtBbox_arrow.pdf} \\
%     \includegraphics[width=0.3\linewidth]{Images/video_4_keyframe.pdf} &
%     \includegraphics[width=0.3\linewidth]{Images/video_4_gtBbox_arrow.pdf} &
%     \includegraphics[width=0.3\linewidth]{Images/video_4_dtBbox_arrow.pdf} \\
%     $t$ & $t+1 \colon t+4$ & $t+1 \colon t+4$ 
%     \end{tabular}
%     \caption{ 
%     \textbf{[H1]: Trajectory anticipating on MovingDigits.} We show time-accumulated frames of digits 6 and 4. Each digit class has an associated linear motion (green arrow). We evaluate trajectory forecasting from a single image on the \textsc{Test-simil} videos where the motion is similar to the training videos, and on the \textsc{Test-diff} videos which have different motion than trained on.  Computing the average IoU@[0.50:.05:0.95] for the forecasts (orange boxes) shows that our model can predict trajectories from a static frame, if similar trajectories are observed in the training set. 
%     %The moving directions of digit 6 and digit 4 as well as their bounding-box detection are the same with that in the training. 
%     %The moving directions of digit 6 and digit 4 are different from that in the training set. 
%     %Regardless of the test set, the bounding-box predictions still follow the directions the corresponding digits have in the training set. 
%     %Our model learns to associate object appearance with motion. 
%     %\fkn{The figure is beautiful. However, it is a bit confusing if you don't read the caption. For example, for digit 4 is it not clear the digit moves in the same direction as of the training set. If you get time, you may change the figure with the trajectory line.}
%     }
%     \label{fig:h1}
% \end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
    \centering
    \begin{tabular}{ccc}
    \small{Input frame} & \small{GT Bbox} & \small{Predicted Bbox} \\
    \includegraphics[width=0.3\linewidth]{Images/video_6_keyframe.pdf} & 
    \includegraphics[width=0.3\linewidth]{Images/video_6_gtBbox_.pdf} &
    \includegraphics[width=0.3\linewidth]{Images/video_6_dtBbox_.pdf} \\
    \includegraphics[width=0.3\linewidth]{Images/video_4_keyframe.pdf} &
    \includegraphics[width=0.3\linewidth]{Images/video_4_gtBbox_.pdf} &
    \includegraphics[width=0.3\linewidth]{Images/video_4_dtBbox_.pdf} \\
    $t$ & $t \colon t+3$ & $t \colon t+3$ \\
    % Avg IoU: & 1.00 & 0.95 
    \end{tabular}
    \caption{ \small
    \textbf{[H1]: Trajectory anticipation on MovingDigits.} We show a single static input frame of digits 6 and 4 and their time-accumulated ground truth and predicted bounding boxes in timesteps $t \colon t+3$. Each digit class has an associated linear motion (green arrow). The match of our predicted bounding boxes and the ground truth bounding boxes shows that our model can predict trajectories from a static frame. 
    %The moving directions of digit 6 and digit 4 as well as their bounding-box detection are the same with that in the training. 
    %The moving directions of digit 6 and digit 4 are different from that in the training set. 
    %Regardless of the test set, the bounding-box predictions still follow the directions the corresponding digits have in the training set. 
    %Our model learns to associate object appearance with motion. 
    %\fkn{The figure is beautiful. However, it is a bit confusing if you don't read the caption. For example, for digit 4 is it not clear the digit moves in the same direction as of the training set. If you get time, you may change the figure with the trajectory line.}
    }
    \label{fig:h1}
\end{figure}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% \begin{table}
%     \centering
%     \begin{tabular}{l c}
%     \toprule
%     & avg IoU ($\uparrow$) \\ \midrule
%     \textsc{Test-Simil} & 0.94 \\
%     \textsc{Test-Diff} & 0.55 \\
%     \bottomrule
%     \end{tabular}
%     \caption{
%         \textbf{[H1]: Evaluating of the forecasted bounding-boxes.}
%         We calculate the average $L_1$ distances and IoU scores between the forecasted bounding-box and the ground truth boxes for both \textsc{Test} and \textsc{Test-diff} sets. 
%         Where the motion remains consistent, our model learns to correcly predict it.
%     }
%     \label{tab:h2}    
% \end{table}

% \begin{table}
%     \centering
%     \resizebox{.7\linewidth}{!}{%
%     \begin{tabular}{c c c c}
%     \toprule
%       \multicolumn{2}{c}{avg $L_1$ ($\downarrow$)} & \multicolumn{2}{c}{avg IoU ($\uparrow$)} \\ \cmidrule(lr){1-2}\cmidrule(lr){3-4}
%         \textsc{Test} & \textsc{Test-diff} & \textsc{Test} & \textsc{Test-diff} \\ \cmidrule(lr){1-2}\cmidrule(lr){3-4} 
%         0.0042 & 0.0126 & 0.94 & 0.55 \\
%     \bottomrule
%     \end{tabular}}
%     \caption{ \small
%         \textbf{[H2]: Quality of the forecasted bounding-boxes.}
%         We calculate the average $L_1$ distances and IoU scores between the forecasted bounding-box and the ground truth boxes for both \textsc{Test} and \textsc{Test-diff} sets. 
%         Where the motion remains consistent, our model learns to correcly predict it.
%     }
%     \label{tab:h2}
% \end{table}

%----------------------------------------------------------------------
\medskip\noindent\textbf{[H2]: Anticipating improves static detection.} The motion cues in-between the static keyframes offer an additional source of supervision. Here, we investigate how the motion anticipating affects the static object detector where we evaluate at test-time on keyframes only.


We explore what types of motion to predict between the static keyframes. %To do so, we evaluate static keyframe detection and vary the motion types used for supervising trajectory forecasting. 
%In our experiments with MovingDigits dataset, we observe that the precision of keyframe detection is improved by our method.
%We conduct experiments on the MovingDigits dataset where the input keyframes are fixed accros all experiments at training and test time, and only the bounding box annotations differ.
%We hypothesize that trajectory motion fore
We consider four types of motion supervision for predicting box trajectories: (1) \textit{Ground truth motion}: trained on true bounding-box trajectories annotated at every frame; (2) \textit{Simulated smooth motion}:  bounding boxes move between keyframes according to a smooth parabola. (Details and examples are in the supplementary material); (3) \textit{Randomized positions}: there is motion, but it is not smooth, the boxes in-between the keyframes can occur at any random position in the image; (4) \textit{No motion}: without motion prediction, \ie, the static object detector baseline trained at every video frame. 

% Another factor \jvg{What is the motivation for evaluating velocity in the "self-supervision" paragraph? }  to consider is the object velocity. A faster object will move a longer distance between frames.  To evaluate velocity, we create and evaluate on three variants of the MovingDigits where the only variable that changes is the velocity (pixels/frame) of the moving digits, where a digit 'bounces back' if it would move outside the frame.


%For each video in the randomized positions variant, the keyframes are the same with the ones in the MovingDigits dataset.
%We only create the frames between each two keyframes to have digits appearing in any randomized locations.
%Similarly, the fake smooth motion variant also has the exactly same keyframes with the MovingDigtis dataset, only the intermediate frames have digits moving in a smooth and continuous trajectory.
%In practice, we choose the fake smooth motion to be a parabola as it is continuous and can connect every two neighbouring keyframes.
%We train our model with the MovingDigits dataset and its two variants separately, and test each of the trained models only on keyframes of the MovingDigits dataset to get the accuracy of keyframe detection.
%We show a figure \xl{add figure of movement} that illustrates how an digit movement of these two variance differs from the linear motion.
%Here the velocity means the number of pixels the digit will move from the current frame to the next frame.

\tab{smoothandcontinuity} shows the keyframe mAP scores for IoU@[0.50:.05:0.95]. 
% \jvg{This also seemed to confuse reviewers to say that "our method does not generalize", because the graph goes down. }
The \textit{No motion} static object detector is the baseline, which uses no motion.
%And even though randomized positions dataset add extra supervision in our method by using the randomized digit locations, it does not improve the performance of keyframe detection over images detector Faster-RCNN.
The \textit{Randomized positions} as supervision is detrimental for object detection because the motion is random, and unpredictable. 
This likely overfits to the random position prediction on the training set, which negatively affects the static detections as well.
%We observe object location prediction is much worse than that for the ground truth motion and even fake smooth motion.
Interestingly, both \textit{Ground truth motion} and \textit{Simulated smooth motion} motion supervision improve the static keyframe detection. We analyzed the results, and notice an improvement in the IoU. 
We speculate that the anticipating loss encourages detecting static regions that are most likely to move coherently, with consistent motion offsets: i.e. same direction.
We conclude that, for non-random motions, adding motion anticipating as an additional source of supervision improves static object detection at keyframes, even when we do not use the ground truth motion between keyframes.
%, even when only sparse keyframes are annotated and the ground truth motion between keyframes is not available \slp{This concl is not true, because the "no motion supervision" is actually "all motion supervision" -- i.e. it's trained at every frame, not sparsely. It's only evaluated sparsely}. 

% \begin{figure}
%     \centering
%     \includegraphics[width=1.\linewidth]{Images/motion_and_continuity.pdf}
%     \caption{ \small
%     \textbf{[H2] Influence of motion forecasting on static object detection.} 
%     % \jvg{You didnt run this on the normal MovingDigits with 2 px/frame?}
%     % \xl{I'm going to run the experiments with 2px/frame}
%     Static keyframe detection mAP on MovingDigits for varying digit velocities (pixels/frame) and motion type supervision.
%     For moderate velocities, and non-random motions, adding motion forecasting improves static object detection at keyframes.
%     % \jvg{Please remove "ours" from fig legend} \jvg{Change the order of the legend so that it reduces the quality, so make it: "Ground truth motion"; "Fake smooth motion"; "Randomized positions"; "No motion supervision". } \jvg{Maybe put a box around the legend? (matplotlib has such an option)} \jvg{x-axis: "velocity (pixel)" = "velocity (pixels/frame)"}
%     }
%     \label{fig:smoothandcontinuity}
% \end{figure}
%=========================================================================================

\begin{table}[]
    \centering
    \resizebox{0.8\linewidth}{!}{%
    \begin{tabular}{lc}
    \toprule
        Motion & Keyframe mAP (\%)  \\ \midrule  
         Randomized positions &  62.68\\
         No motion &  73.51\\
         Simulated smooth motion &  76.57\\
         Annotated motion & 79.31\\
    \bottomrule
    \end{tabular}}
    \vspace{1.5ex}
    \caption{ \small
    \textbf{[H2] Influence of motion anticipating on static object detection.} 
    Static keyframe detection mAP on MovingDigits for varying motion type supervision.
    For non-random motions, adding motion anticipating improves static object detection at keyframes.
    }
    \label{tab:smoothandcontinuity}
\end{table}



%=========================================================================================

\subsection{Ablation of model components}
We run all ablation experiments on an ImageNet VID \cite{ILSVRC15} subset containing the classes `dog', `giant\_panda', and `hamster'. We use a ResNet-101 for feature extraction.
%- Subset of ImageNetVid (e.g. 10 classes):
% \clearpage

%--------------------------------------------------------------------
\smallskip\noindent\textbf{[A1]: The effect of the trajectory loss.}
We evaluate  each term in our trajectory loss $L_\text{traj} = L_{\sum} + L_{\text{bag}(\delta)}$ in \eq{traj-loss}, compared to the standard loss $L_{\text{bag}}$ in \eq{loss}. 
The mAP scores for trajectory lengths $T{=}4$ and $T{=}8$ are in \tab{loss_comparison}.
The $L_\text{traj}$ loss has a higher mAP than the bag loss $L_{\text{bag}}$ for both trajectory lengths.
$L_\text{traj}$ enforces continuity and smoothness in the predictions over time thus leads to more precise predictions.
Furthermore, the improvement of $L_\text{traj}$ over $L_{\text{bag}}$ is larger for longer trajectories, e.g. for $T{=}4$ and $T{=}8$, $L_\text{traj}$ outperforms $L_{\text{bag}}$ by 1.66\% and 2.18\% respectively.
Our $L_\text{traj}$ loss is defined using offsets, without offsets the $L_{\sum}$ would be equivalent to $L_{\text{bag}}$. 
We observe that the effect of predicting offsets between neighboring boxes $\delta_{t+l}$, instead of bounding-box coordinates $B_{t+l}$ gives an improvement of 0.81\% and 0.89\%. 
When considering $L_{\text{bag}(\delta)}$ or $L_{\sum}$ individually, their mAP is lower or on par with $L_\text{traj}$.
This is because $L_{\text{bag}(\delta)}$ cannot enforce trajectory continuity, while $L_{\sum}$ cannot ensure that trajectories do not diverge by accumulating errors over time.  
%constrains the cumulative pairwise distances from frame $t$ up to every frame $t+l$ add up to the ground truth distance, which only address the continuity of the predicted trajectory but trajectory between frame $t$ and frame $t+l$ can be randomly connected.
Predicting offsets instead of box coordinates results in better accuracy.
\begin{table}
    \centering
    \resizebox{0.7\linewidth}{!}{%
    \begin{tabular}{l c c}
    \toprule
                                    & \multicolumn{2}{c}{Trajectory  length (mAP \%) }\\ \cmidrule(lr){2-3}
        Loss                        & T=4                & T=8  \\ \midrule
        \textbf{$L_{\text{bag}}$}   & 87.54 $\pm$ 0.16   & 83.97 $\pm$ 0.71  \\ \midrule
        $L_{\sum}$                  & 87.95 $\pm$ 0.27   & 84.09 $\pm$ 0.67 \\
        $L_{\text{bag}(\delta)}$    & 85.19 $\pm$ 0.66   & 79.73 $\pm$ 1.01 \\
        $L_\text{traj}$    &  \textbf{89.20 $\pm$ 0.21}  & 86.15 $\pm$ 0.75 \\
        %$L_{\Delta}$ (with boxes)   &  88.39 $\pm$ 0.30  & 85.26 $\pm$ 0.69 \\ 
        %$L_{\Delta}$ (with offsets) &  \textbf{89.20 $\pm$ 0.21}  & 86.15 $\pm$ 0.75 \\ 
    \bottomrule
    \end{tabular}}
    \vspace{1.5ex}
    \caption{ \small
    \textbf{[A1]: Loss choice.}
    Compared to $L_{\text{bag}}$, the $L_{\text{bag}(\delta)}$ loss does worse, whereas $L_{\sum}$ performs on par. Their combination in  $L_\text{traj} = L_{\sum} + L_{\text{bag}(\delta)}$  outperforms $L_{\text{bag}}$.
    Predicting offsets instead of bounding-box coordinates in the trajectory network gives better results.
    These patterns are consistent over both trajectory lengths. 
    }
\label{tab:loss_comparison}
\end{table}

%----------------------------------------------------------------------
\medskip\noindent\textbf{[A2]: The effect of the sparse annotation loss.}
We test our model using the $L_\text{traj}^{\text{(sa)}}$ loss for sparse annotations.
To evaluate this in a controlled setting, we sub-sample keyframe annotations from the fully annotated ImageNet VID subset to mimic a sparse annotation scenario, and evaluate only on keyframes. 
We compare ground truth motion result with the result of anticipating linearly interpolated trajectories between keyframes.
\tab{a2-sa} shows that the $L_{\text{bag}(\delta)}^{\text{(sa)}}$ component does not contribute much for the keyframe detection.
This is because $L_{\text{bag}(\delta)}^{\text{(sa)}}$ constrains the predicted offsets to match the pairwise offsets of the pseudo trajectory at every frame, which is not useful here since the motion is simulated.
The $L_{\sum}^{\text{(sa)}}$ component performs on par with the $L_\text{traj}^{\text{(sa)}}$.
And the keyframe detection accuracy with the sparse annotation loss $L_\text{traj}^{\text{(sa)}}$ is close to that with the proposed fully-supervised loss $L_\text{traj}$.
%In later experiments we use $L_{\Delta(SS)} = L_{obj(SS)}$. \jvg{I dont find this very convincing, because $L_{\Delta(SS)}$ is the best.. Can we think of another reason? (at least we should start the YouTube BB exp with the $L_{\Delta(SS)}$ loss after the deadline. }

\begin{table}
    \centering
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{l c c c c}
    \toprule
        & \multicolumn{4}{c}{Keyframe mAP\%}\\ \cmidrule(lr){2-5}
        & \multirow{2}{*}{$L_\text{traj}$} & \multicolumn{3}{c}{Sparse annotation loss}\\ \cmidrule(lr){3-5}
                  &   & $L_{\sum}^{\text{(sa)}}$ &  $L_{\text{bag}(\delta)}^{\text{(sa)}}$ &  $L_\text{traj}^{\text{(sa)}}$ \\ \midrule           
        T=4     &  91.03 $\pm$ 0.19 & 90.35 $\pm$ 0.34 & 74.61 $\pm$ 0.72 & 90.76 $\pm$ 0.26 \\             
        T=8     &  87.94 $\pm$ 0.66 & 86.98 $\pm$ 0.73 & 68.76 $\pm$ 0.99 & 87.12 $\pm$ 0.69 \\
    \bottomrule
    \end{tabular}}
    \vspace{0.05ex}
    \caption{ \small
    \textbf{[A2]: Sparse annotation loss analysis.}
    We sub-sample keyframes of the fully annotated ImageNet VID subset to mimic the sparse annotations, and evaluate our sparse annotation loss on keyframe detection. 
    The $L_{\text{bag}(\delta)}^{\text{(sa)}}$ does not improve the detection accuracy, while $L_{\sum}^{\text{(sa)}}$ performs on par with the $L_\text{traj}^{\text{(sa)}}$. 
    The sparse annotation loss achieves a comparable accuracy on keyframe detection with our fully-supervised loss $L_\text{traj}$.
    }
\label{tab:a2-sa}
\end{table}

\begin{comment}
\begin{table}
    \centering
    \resizebox{0.8\linewidth}{!}{%
    \begin{tabular}{l c c}
    \toprule
                                    & \multicolumn{2}{c}{Trajectory  length (Keyframe mAP\%) }\\ \cmidrule(lr){2-3}
        Loss                                       & T=4                & T=8  \\ \midrule
        $L_\text{traj}$                   & 91.03 $\pm$ 0.19        & 87.94 $\pm$ 0.66 \\ \midrule
        $L_{\sum}^{\text{(ss)}}$                   & 90.35 $\pm$ 0.34        & 86.98 $\pm$ 0.73 \\[5px] 
        $L_{\text{bag}(\delta)}^{\text{(ss)}}$     & 74.61 $\pm$ 0.72        & 68.76 $\pm$ 0.99 \\[5px]
        $L_\text{traj}^{\text{(ss)}}$     & 90.76 $\pm$ 0.26        & 87.12 $\pm$ 0.69 \\ 
    \bottomrule
    \end{tabular}}
    \vspace{0.05ex}
    \caption{ \small
    \textbf{[A2]: Self-supervised loss analysis.}
    We sub-sample keyframes of the fully annotated ImageNet VID subset to mimic the sparse annotations, and evaluate our self-supervised loss on keyframe detection. 
    The $L_{\text{bag}(\delta)}^{\text{(ss)}}$ does not improve the detection accuracy, while $L_{\sum}^{\text{(ss)}}$ performs on par with the $L_\text{traj}^{\text{(ss)}}$. 
    The self-supervised loss achieves a comparable accuracy on keyframe detection with our fully-supervised loss $L_\text{traj}$.
    }
\label{tab:a2-ss}
\end{table}
\end{comment}
%----------------------------------------------------------------------
\begin{comment}
\medskip\noindent\textbf{[A3]: The effect of trajectory length.}
We test how long the forecasted object trajectories can be before substantial precision shrinkage. 
We consider trajectory lengths: $T \in \{4,8,16,32\}$.
%- How long is the trajectory before results get worse (4, 10 frames)
%We use the number of frames ($T$) to represent the length of trajectory.
\tab{trajectory_length} shows that mAP reduces as as the trajectory length increases.
For trajectories longer than $T=16$, there is a noticeable drop in detection accuracy.
Our method relies on smooth and continuous object trajectories.
However, when the trajectory is too long, the object motion may vary or the object may leave the frame or new object may enter the frame. 
These changes result in the decrease of our model\lq s performance.

\begin{table}[]
    \centering
    \resizebox{.95\linewidth}{!}{%
    \begin{tabular}{c c c c}
    \toprule
       \multicolumn{4}{c}{Trajectory length (mAP \%)}\\ \midrule
       {T=4} & {T=8} & {T=16} & {T=32}\\ \midrule 
       89.20 $\pm$ 0.21 & 86.15 $\pm$ 0.75 & 77.69 $\pm$ 0.95& 60.08 $\pm$ 1.25\\
    \bottomrule
    \end{tabular}}
    \caption{ \small
        \textbf{[A2]: Trajectory length.}
        The trajectory length our method can forecast before substantial precision shrinkage. The mAP decreases as the trajectory length increases, and a length of 16 is where the model fails to be accurate.
    }
    \label{tab:trajectory_length}
\end{table}
\end{comment}

%----------------------------------------------------------------------
\medskip\noindent\textbf{[A3]: Inference speed vs. accuracy trade-off.}
%\xl{I'm thinking add a graph of speed-trajectory length-accuracy trade-off here to replace the \textbf{[A2]}. What would you suggest?} \jvg{sounds good; can you try a version?}\fkn{Section A2 is good. Why remove it? What do you mean spead-trajectory and length-accuracy?}
We can control the inference speed by sampling fewer keyframes, and thus predicting longer trajectories.


We analyse the speed vs. accuracy trade-off of our method on the subset of ImageNet VID.
\fig{speed-acc} shows we can reach an mAP of 89.2\% with a runtime of 39.6 FPS.
Moreover a noticeable drop in mAP occurs at trajectories longer than 10 frames.
However, when the trajectory is too long, the object motion may vary or the object may leave the frame or new object may enter the frame. 
These changes result in the decrease of our model\rq s performance.
The prediction trajectory length can be chosen according to the speed-accuracy trade-off.

\begin{figure}
    \centering
    \includegraphics[width=1.\linewidth]{Images/speed_trajectory_acc.pdf}
    \caption{ \small
    \textbf{[A3] Inference speed vs. accuracy trade-off.}
    We can increase inference speed (FPS) by sampling fewer keyframes and predicting longer trajectories. Yet, with increasing trajectory length the mAP decreases. 
    The prediction trajectory length can be chosen according to the required speed-accuracy trade-off.
    }
    \label{fig:speed-acc}
\end{figure}

%----------------------------------------------------------------------
%\medskip\noindent\textbf{[A5]: The effect of the object detection backbone.}
%If time allows it, another object detection backbone would be great: SSD, Yolo

%------------------------------------------------------------------
\subsection{State-of-the art comparisons}
\medskip\noindent\textbf{[S1]: Experiments on ImageNet VID.}
We compare our method with state-of-the-art video object detection methods on ImageNet VID  in \tab{ImageNetVID} using a ResNet-101 as the feature extractor.
We mark methods without post-processing with \cmark.
Methods with post-processing add extra computational cost.
Our method does not use any post-processing.
%, nor does it rely on feature aggregation of region proposals \jvg{Confusing. Why is this good/bad?}.
We use a prediction trajectory of length $T{=}4$, as this already allows a considerable reduction in computation speed.
Among all methods, our method is the most accurate with a 87.2\% mAP, which has a 2.7\% improvement over the leading MEGA \cite{chen2020memory}.
We also report runtime (FPS) and train-time (hrs/epoch) to show that our method is fast and efficient.
We measure the efficiency using the code provided by the original papers, and where the code is not available we mark this with `-'. 
%Due to the unavailability of code at the time of experiments, except those methods marked with '-', we measure the training time per epoch and inference time from the code provided by the original papers.
Note that for the training time this is a rough estimate, when considering the same settings (batch-size, GPU) for all methods. 
We tested the inference runtime speed on a single NVIDIA GTX 1080 Ti.
In terms of both training time and runtime our method is most efficient.
Our method has fast inference time with 39.6 FPS, which is $\approx 1.8\times$ faster than existing fast methods like LWND \cite{jiang2019deformable} and ST-Lattice \cite{chen2018optimizing}.
Our efficiency comes from predicting object locations for the next $T$ frames, while processing only temporally sub-sampled keyframes.

\begin{table}[]
    \centering
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{l@{\hskip -0.05in}c@{\hskip 0.in}c@{\hskip 0.in}c@{\hskip 0.1in}c@{\hskip 0.1in}r@{\hskip 0.1in}r}
    \toprule
        Methods &  Backbone & No Post- & mAP (\%)  & Train-time & Runtime \\ 
         &   & proc. & & (hrs/epoch) & (FPS) \\ \midrule
         Faster-RCNN \cite{ren2015faster}& R101 & \cmark & 73.6 & 1.55 & 21.2\\
         LWND \cite{jiang2019deformable} & R101 & \cmark & 76.3 & - & 20.0\\
         FGFA \cite{zhu2017flow}& R101 &  & 78.4 & 6.59 & 5.0 \\
         THP \cite{zhu2018towards}& R101+DCN & \cmark & 78.6 & - & - \\
         ST-Lattice \cite{chen2018optimizing} & R101 &  & 79.6 & 1.40 & 20.0\\
         D\&T \cite{feichtenhofer2017detect}& R101 &  & 80.2 & 6.56 & 5.0\\
         MANet \cite{wang2018fully} & R101 &  & 80.3 & 6.88 & 4.9 \\
         STSN \cite{bertasius2018STSN}& R101+DCN &  & 80.4 & - & -\\
         STMN \cite{xiao2018STMN}& R101 &  & 80.5 & 2.49 & 13.2\\
         TROI \cite{gong2021temporalROI} &  R101 &  & 80.5 & 5.18 & 6.4\\
         SELSA \cite{wu2019sequence}& R101 &  & 80.5 & 3.15 & 10.6 \\
         OGEMN \cite{deng2019OGEMN} & R101+DCN &  & 81.6 & - & 8.9\\
         SparseVOD \cite{hashmi2022spatio}& R101 & \cmark & 81.9 & - & 14.4\\
         BoxMask \cite{hashmi2022boxmask} & R101 & \cmark & 83.2 & - & 6.1\\
         RDN \cite{deng2019RDN}& R101 &  & 83.8 & - & -\\
         HVRNet \cite{han2020mining}& R101 &  & 83.8 & -& -\\
         TF-Blender \cite{cui2021tf}& R101 & \cmark & 83.8 & - & 4.9\\
         MEGA \cite{chen2020memory}& R101 &  & 84.5 & 6.34 & 5.3 \\\midrule
         TransVOD \cite{zhou2022transvod} (Deformable DETR) & R101 & \cmark &81.9 & - &32.3 \\
         PTSEFormer \cite{wang2022ptseformer} (Deformable DETR) & R101 &\cmark &88.1 & - & -\\
         TransVOD \cite{zhou2022transvod} (Deformable DETR) & SwinB & \cmark&90.1 & -&14.9 \\
         \midrule
         Ours (Faster RCNN) & R101 & \cmark & 87.2 & 0.78 & \textbf{39.6}\\
         Ours (Deformable DETR) & R101 & \cmark & 87.9 & -&36.4 \\
        Ours (Deformable DETR) & SwinB & \cmark & \textbf{91.3} & -&18.1 \\
    \bottomrule
    \end{tabular}}
    \caption{ \small
    \textbf{[S1]: Experiments on ImageNet VID.}
    We indicate the methods without video-level post-processing (e.g. SeqNMS, Tube Rescoring, BLR) with \cmark in the table. 'No Post-proc.' means no post-processing. R101 here is ResNet-101. The runtime is measured on a NVIDIA GTX 1080 Ti. 
    Our method achieves the best performance and fastest runtime among all the methods using two-stage detectors (e.g. Faster RCNN).
    With a stronger detector and backbone, our method is on par with PTSEFormer and better than TransVOD.}
    \label{tab:ImageNetVID}
\end{table}

Because our method is detector agnostic, we also compared our method with methods using more advanced detectors, Deformable DETR \cite{zhu2020deformable}, and more advanced backbone SwinB \cite{liu2021swin}. We showed ImageNet VID results in \tab{ImageNetVID}. Our method achieves on-par results with PTSEFormer \cite{wang2022ptseformer} with the Deformable DETR detector and R101 backbone, and our method improves overall state-of-the-art with a SwinB backbone.

% \begin{table}[h]
% {
% \centering
%     \resizebox{1\linewidth}{!}{%
%     \begin{tabular}{l@{\hskip 0.1in}c@{\hskip 0.1in}c@{\hskip 0.1in}c@{\hskip 0.1in}r}
%     \toprule
%         Methods & Base Detector & Backbone & mAP (\%) & Runtime (FPS)\\
%         \midrule
%         TransVOD \cite{zhou2022transvod} & Deformable DETR & R101 & 81.9 & 32.3 \\
%         PTSEFormer \cite{wang2022ptseformer} & Deformable DETR & R101 & 88.1 & - \\
%         TransVOD \cite{zhou2022transvod} & Deformable DETR & SwinB & 90.1 & 14.9 \\
%         \midrule
%         Ours & Faster-RCNN & R101 & 87.2 & 39.6 \\
%         Ours & Deformable DETR & R101 & 87.9 & 36.4 \\
%         Ours & Deformable DETR & SwinB & 91.3 & 18.1 \\
%     \bottomrule
%     \end{tabular}}
% }
%    \caption{ \small
%    \textbf{[S1]: Experiments on ImageNet VID.} Our method is the new state-of-the-art with a stronger detector and backbone, on par with PTSEFormer and better than TransVOD with a stronger detector and backbone. 
%    \slp{Could you merge this with the prev table}
%    }
%    \label{tab:advanced_detector_backbone}
%    \vspace{-10px}
% \end{table}

%-----------------------------------------------------------------------
\medskip\noindent\textbf{Comparison on different motion speeds.} We also compare on different motion speeds with other methods as shown in \tab{ImageNetVID_speed}.
The category of object motion speeds in ImageNet VID follows FGFA \cite{zhu2017flow}.
Our method improves mAP significantly on slow and medium motion speeds and achieves comparable results to the previous best method on fast motion speed, which shows the effectiveness of our method across different motion speeds.

~\\

\begin{table}[]
    \centering
    \resizebox{1\linewidth}{!}{%
    \begin{tabular}{l@{\hskip 0.1in}c@{\hskip 0.1in}c@{\hskip 0.1in}c@{\hskip 0.1in}r@{\hskip 0.1in}r}
    \toprule
        Methods & Backbone & mAP (\%)  & mAP (\%) & mAP (\%) & mAP (\%) \\  
        & & & (slow) & (medium) & (fast) \\ \midrule
         FGFA \cite{zhu2017flow} & R101 & 78.4 & 83.5 & 75.8 & 57.6 \\
         MANet \cite{wang2018fully} & R101 & 80.3 & 86.9 & 76.8 & 56.7 \\
         SELSA \cite{wu2019sequence}& R101 & 80.5 & 86.9 & 78.9 & 61.4 \\
         OGEMN \cite{deng2019OGEMN} & R101+DCN & 81.6 & 86.2 & 78.7 & 61.1\\
         HVRNet \cite{han2020mining} & R101 & 83.8 & 88.7 & 82.3 & \textbf{66.6} \\
         IFFNet \cite{jin2022feature} & R101 & 79.7 & 87.5 & 78.7 & 60.6 \\\midrule
         Ours & R101 & \textbf{87.2} & \textbf{92.2} & \textbf{86.1} & 66.5\\
    \bottomrule
    \end{tabular}}
    \caption{ \small
    mAP on ImageNet VID across different motion speeds. 87
    Our method improves mAP on different motion speeds.}
    \label{tab:ImageNetVID_speed}
\end{table}


%-----------------------------------------------------------------------
\medskip\noindent\textbf{[S2]: Experiments on EPIC KITCHENS-55.} In EPIC KITCHENS-55, each frame contains avg/max 1.7/9 objects, which is more challenging compared to ImageNet VID. The Epic Kitchens video object detection task consists of 32 different kitchens and 290 classes. The training set has 272 video sequences captured in 28 kitchens. For evaluation, 
106 sequences collected in the same 28 kitchens (S1) and 54 sequences collected in 4 other unseen kitchens (S2) are used. 
We use a prediction trajectory length of $T{=}4$ and evaluate for two IoU thresholds of 0.5 and 0.75.

As summarized in \tab{EPIC-kitchens}, our method is more accurate than previous state-of-the-art methods for both Seen/Unseen splits.
%\slp{What are these seen unseen splits?}
This indicates that our method is applicable to more complex video detection tasks.
%\slp{What makes these videos complex compared to ImageNet VID?}

\begin{table}
    \centering
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{l@{\hskip -0.05in}r@{\hskip 0.1in}r r@{\hskip 0.1in}r}
    \toprule
          & \multicolumn{2}{c}{S1} &  \multicolumn{2}{c}{S2}\\ \cmidrule(lr){2-3}\cmidrule(lr){4-5}
         Methods & mAP@.5 & mAP@.75 & mAP@.5 & mAP@.75 \\  \midrule
         EPIC \cite{damen2018scaling}& 34.2 & 8.5 &  32.0 & 7.9\\
         Faster-RCNN \cite{wu2019sequence}& 36.6  & 9.9 &  31.9 & 7.4\\
         SELSA \cite{wu2019sequence}& 37.9 & 9.8  & 34.8 & 8.1\\
         SELSA-ReIm + TROI \cite{gong2021temporalROI} &  42.2 & - & 39.6 & - \\
         BoxMask \cite{hashmi2022boxmask} & 44.3 & 18.5 &  41.3  & 15.7 \\\midrule
         Ours & \textbf{44.9} & \textbf{18.7} &  \textbf{41.7} & \textbf{16.0}\\
    \bottomrule 
    \end{tabular}}
    \caption{ \small
    \textbf{[S2]: Experiments on EPIC KITCHENS-55.}
    S1 and S2 represent Seen and Unseen splits respectively. 
    Our method achieves promising results for both test sets and IoU thresholds.}
    \label{tab:EPIC-kitchens}
\end{table}

%-----------------------------------------------------------------------
\subsection{Sparsely annotated videos} 
%We run the Faster-RCNN \cite{ren2015faster} object detector on YouTube-BoundingBoxes dataset \cite{real2017youtube}. 
\begin{table}[]
    \centering
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{l c c c}
    \toprule
        Methods & Keyframe step & Label step & mAP (\%) \\ \midrule
         Faster-RCNN \cite{ren2015faster}                & 60 & 60 & 47.6\\ 
         Faster-RCNN \cite{ren2015faster}                & 30 & 30 & 58.7\\ \midrule
         Ours $L_\text{traj}$ \vspace{2px}               & 60 & 30 & 51.3 \\ \cdashline{1-4}
         Ours $L_\text{traj}^{\text{(sa)}}$              & 30 & 1 & \textbf{59.8}\\
    \bottomrule
    \end{tabular}}
    \caption{ \small
    \textbf{Sparsely annotated data.}
    We report mAP on the sparsely annotated YouTube-BoundingBoxes. 
    The sparse annotation loss $L_\text{traj}^{\text{(sa)}}$ using interpolated pseudo trajectory labels improves keyframe detection.
    Our method outperforms Faster R-CNN by making effective use of annotations, even if these are not present in the dataset. 
    }
    \label{tab:YouTube-BoundingBoxes}
\end{table}

%%%%%%%%%

%%%%%%%%%


The YouTube-BoundingBoxes dataset has sparse annotations: the video frame rate is 30 frames per second, and on average it only has annotations at 1 fps. 
We evaluate our method compared to the Faster R-CNN \cite{ren2015faster} baseline on YouTube-BoundingBoxes in \tab{YouTube-BoundingBoxes}.
The networks receive as input keyframes sampled with a step 60 and 30, which is every 60 frames and 30 frames in the video, respectively.
During training, for the Faster R-CNN we use the labels at the keyframes, while for our method we use labels with a step of 30 or 1 over the input keyframes. 
For a label step of 30 and a keyframe step of 60, we use 2$\times$ more labels than input frames, while for a label step of 1 and keyframe step of 30, we use 30$\times$ more labels than frames. 
%Since the annotation is sparse, we interpolate the trajectory between every two annotated frames as a even speed parabola and create pseudo labels (pseudo bounding box ground truth) for every frame in between, which make label step 1.
Since the video annotations are sparse we do not have labels at every frame, therefore for a label step of 1, we use our sparse annotation loss.
For the $L_\text{traj}^\text{(sa)}$ we define the box trajectories to be linearly interpolated pseudo trajectories.
For keyframes sampled with a step of 60, our method achieves higher accuracy than Faster R-CNN by using $2\times$ more labels, while processing the same input keyframes.
% which shows that our method learns the temporal information and continuity by predicting object locations, even it is just predicting one frame further here.
%We also show that with the proposed self-supervised loss, we can observe that imposing piecewise continuity over time is sufficient on its own for improving keyframe detection.
With the same input keyframes every 30 frames, our method even achieves a 1.1\% higher mAP than Faster R-CNN while optimizing a simulated motion between these frames.
This result indicates that the precise location of an object along a trajectory is not essential for keyframe detection. 
% \fkn{The slow, fast table is missing. The one from cvpr rebuttal. I think it is good to highlight that method can handle slow and fast motion. } \xl{the table is there, see above.}
%We can create a smooth and continuous pseudo trajectory to boost keyframe detection.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
\subsection{Method limitations}



Despite our state-of-the-art results, with successful predictions as in \fig{examples}(a), we also identify several limitations.
In practice, multiple motion patterns can be associated with the exactly same appearance: e.g people can walk or jump.
If a specific object's appearance contains multiple motion patterns, our method may fail to predict the correct object locations.
%But in this case, our method may use different background features to distinguish between multiple motion patterns even if the object appearance is the same, unless the background is also the same.
Another failure case is if objects appear or disappear in the middle of a trajectory. In these cases, we will either miss the objects or over-predict.
Yet another limitation of our method is the assumption that the motion changes smoothly. 
If the object trajectories have extremely large variations in a short timestep because of the video frame rate, or other reasons, for example, the dog in \fig{examples}(b) suddenly changed its moving direction, our trajectory network may not be able to learn such complex motion patterns.
We might miss some detection of intermediate frames as shown in \fig{examples}(b), but our method can recover the detection by the next keyframe detection. While these hypothetical limitations might exist, they can only influence our method minimally, since we miss only a few hundred milliseconds, which is reflected in our state-of-the-art results compared to other methods for video object detection. 

%- \fkn{The assumption was that appearance doesn't change a lot. So the large change of appearance might be a limitation.} \slp{of appearance is for the detector not for us}

\begin{figure}[t]
    \centering
    \begin{tabular}{cc}
        \includegraphics[trim={5cm 0cm 5cm 0cm},clip,width=.45\linewidth]{Images/output1450.jpg} &
        \includegraphics[trim={5cm 0cm 5cm 0cm},clip,width=.45\linewidth]{Images/output1.jpg} \\ 
        \includegraphics[trim={5cm 0cm 5cm 0cm},clip,width=.45\linewidth]{Images/output1452.jpg} &
        \includegraphics[trim={5cm 0cm 5cm 0cm},clip,width=.45\linewidth]{Images/output2.jpg} \\ 
        \includegraphics[trim={5cm 0cm 5cm 0cm},clip,width=.45\linewidth]{Images/output1455.jpg} &
        \includegraphics[trim={5cm 0cm 5cm 0cm},clip,width=.45\linewidth]{Images/output3.jpg} \\ 
        \includegraphics[trim={5cm 0cm 5cm 0cm},clip,width=.45\linewidth]{Images/output1456.jpg} &
        \includegraphics[trim={5cm 0cm 5cm 0cm},clip,width=.45\linewidth]{Images/output4.jpg} \\ 
        \includegraphics[trim={5cm 0cm 5cm 0cm},clip,width=.45\linewidth]{Images/output1457.jpg} &
        \includegraphics[trim={5cm 0cm 5cm 0cm},clip,width=.45\linewidth]{Images/output5.jpg} \\ 
        %\includegraphics[trim={5cm 0cm 5cm 0cm},clip,width=.5\linewidth]{Images/success7.jpg} &
        %\includegraphics[trim={10cm 4cm 10cm 4cm},clip,width=.5\linewidth]{Images/failure6.jpg} \\ 
        \small{(a) Success case} & \small{(b) Failure case} \\
    \end{tabular}   
    \caption{ \small
        Example predictions. The white boxes are the ground truth. We show one success case in (a) containing a `dog' running at a fast speed. 
        In (b) the failure case shows a `dog' suddenly changes its moving direction, we missed the detection in the third and fourth frames. Yet we recovered the detection in the fifth frame by the keyframe detection.
        When objects move smoothly our detections are accurate, yet when the motion has extremely large variations, the motion is unpredictable, and objects enter and leave the frame, our method fails.
     }
    \label{fig:examples}
\end{figure}

==> Paper/introduction.tex <==
\section{Introduction}

% Problem(s) statement
\fkn{The first paragraph motivation is a bit weak in my opinion. Reviewer could argue this is video object detection, why do you you care about discontinuous object trajectories. What is written here is a hypothesis that VOT methods are not using smoothness and continuous motion information, therefore, they miss detection in some frames. We try to show in this paper that this information improve the result. I feel just adding few words and brushing it makes it more clear.}
\jvg{Ill start rewriting the intro; might take a bit of time... } Objects in videos typically do not appear and disappear randomly.
In fact, video objects have motion patterns that are continuous and smooth over time.
However, current video object detection methods ignore the smoothness of object motion and continuity \cite{chen2018optimizing, han2016seq, kang2016object}, and process the video frames one by one, while using post-processing to add the missing temporal continuity.
While other methods integrate temporal information over sub-sampled frames \cite{wu2019sequence, chen2020memory, cui2021tf, han2020mining, jiang2019deformable}, and thus do not have access to object locations between these sub-sampled frames, and therefore may still miss temporal information.
The missing temporal information can lead to omitted objects and unrealistic, discontinuous object trajectories.

% We add continuity by forecasting
We propose to leverage the continuity of object trajectories over time for video object detection.
Specifically, we hypothesize that we can predict the future motion of an object based on its current position. 
This hypothesis allows us to forecast object locations over time. 
We consider short periods of time, over which it is practical to assume that the object appearance does not change dramatically.
We start from single video frames and anticipate object locations over the next few frames.
By doing so, we integrate the smoothness and continuity of object trajectories, and make temporally-consistent object location predictions.
\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{latex/Images/fig1}
    \caption{ \small
        Forecasting object locations is both temporally consistent and efficient.
        By viewing a video frame $t$ and anticipating the object locations over the following $T$ timesteps, we incorporate temporal consistency and smoothness of object motion.
        Moreover, we are efficient because we do not need to process all video frames, while estimating the location information of all video frames. 
    }
    \label{fig:idea}
\end{figure}

% No missing information and efficiency
To avoid missing information between the sampled video frames and, thus avoid discontinuous object motions, we make use of the object trajectory information at every frame.
Concretely, we uniformly sample from the video a set of frames at a sampling interval $T$, which we call ``keyframes".
For each keyframe, we predict object locations, as shown in \fig{idea}.
Subsequently, for all the in-between frames, we forecast the object locations and optimize these predictions with respect to given object trajectories.
Moreover, because we are interested only in the smoothness of the trajectory, we propose a sparse annotation extension of our method, where we do not need to know the true object trajectories.
For the sparse annotation case we assume the trajectory is defined by a continuous smooth function.
Our method is efficient by only processing the subsampled keyframes through the network, whilst predicting object locations at every frame in the video.
Thus, we circumvent the missing information caused by sampling video frames, while being efficient.

% Contributions
To summarize, this paper makes the following contributions:
(i) We propose an efficient video object detection method that integrates temporal continuity and smoothness in the model, without the need of post-processing;
(ii) Additionally, we can enforce temporal continuity by defining fabricated object trajectories, to replace the true trajectories;  
(iii) We are efficient by only processing keyframes through the network, but we are also complete by using the object location information at all frames, rather than only the sampled frames;
(iv) Our experimental results on ImageNet-VID \cite{ILSVRC15}, EPIC KITCHENS-55 \cite{damen2018scaling}, and YouTube-BoundingBoxes \cite{real2017youtube} show that by predicting object motion from the current keyframe improves accuracy over existing video object detection methods, while being faster at both training and inference time. \fkn{Is it not better to put the most important contribution first? To me, the increase accuracy is more important that efficiency. But I also doubt about changing the order.}
\jvg{Often its best to put the most important ones last, as they are then emphasized the most.}




